Timeliness-Fidelity Tradeoff in 3D Scene Representations

Real-time three-dimensional (3D) scene representations serve as one of the building blocks that bolster various innovative applications, e.g., digital manufacturing, Virtual/Augmented/Extended/Mixed Reality (VR/AR/XR/MR), and the metaverse. Despite substantial efforts that have been made to real-time communications and computing, real-time 3D scene representations remain a challenging task. This paper investigates the tradeoff between timeliness and fidelity in real-time 3D scene representations. Specifically, we establish a framework to evaluate the impact of communication delay on the tradeoff, where the real-world scenario is monitored by multiple cameras that communicate with an edge server. To improve fidelity for 3D scene representations, we propose to use a single-step Proximal Policy Optimization (PPO) method that leverages the Age of Information (AoI) to decide if the received image needs to be involved in 3D scene representations and rendering. We test our framework and the proposed approach with different well-known 3D scene representation methods. Simulation results reveal that real-time 3D scene representation can be sensitively affected by communication delay, and our proposed method can achieve optimal 3D scene representation results.

==> chapters/1_introduction.tex <==
\section{Introduction}
3D reconstuction involves the process of capturing, interpreting, and recreating a three-dimensional representation of an object or a scene from two-dimensional images or sensor data.  By enabling comprehensive understanding and interaction with the visual world. it served as the fundamental building blocks for various emerging applications, e,g, digital manufacturing, robotics, virtual/Augmented/Extended/Mixed Reality (VR/AR/XR/MR), metaverse. For example,  different virtual objects including trees, buildings can be generated from the real-world enities by 3D reconstruction to provide immersive virtual world of the Metaverse,

As the fundamental infrasture to provides services for 3D reconstuction, communication systems have dedicated significant efforts to guarantee both high reliability and low latency. 5G standard has defined the three categories of  communication services, i.e., eMBB, mMTC, and uRLLC. In particular, uRLLC is designed for real-time applications with stringent KPIs on latency (around 1 ms) and reliability (up to 99.99999$\%$). Recently, the fine-grained KPIs for different vertical industries have been released in~\cite{3GPP}. For example, in  motion control systems, the typical KPIs are 99.9999\% availability, 1~ms cycle time, 40–250 bytes typical payload size, and 100 devices per square kilometer. In VR video streaming, the typical KPIs include 1 Gbps (smooth play) or
2.35 Gbps (interactive) data rate to support 10~ms latency for 8K resolution, 120~FPS, and 360~degree visual field VR video steaming~\cite{mangiante2017vr}.
%Nevertheless, It is still cannot fulfill all the Key Performance Indicators (KPIs) in emerging real-time CV applications like self-driving, Virtual/Augmented Reality (VR/AR)~\cite{mangiante2017vr}. 
In the future, the 6G standard would introduce even stringent KPI requirements~\cite{9369424}. 


Although a variety of communication KPIs for different real-time applications have been specified in the 5G standard, the connection between these communication KPIs and the KPI requirements of real-time 3d reconstruction remains unclear. This knowledge gap leads to unprecedented challenges and hinders the emerging of new 3D reconstruction related applications. In addition, communication system design alone is insufficient to tackle the challenges in real-time 3D reconstuction, as the overall system  performance depends on numerous factors beyond communications. These factors include sensing, sampling, computing (inference and rendering), storage, etc. Thus, it is essential to adopt interdisciplinary approaches to address these challenges, where the distinct characteristics of real-time 3d reconstruction-related applications should be considered. 

Rencent study focus on ...

This paper aim seeks to pave the way for investigating the imperfect communication effects on the performance of 3D reconstruction. Specifically, the channel is modelled as the SPP and the neural rendering method is selcted as the 3D influence of packet burstiness and latency on the efficacy of 3D reconstuction. As we know, this is the first paper that investate the communication...



==> chapters/3_system_model.tex <==
\section{System Model}
\subsection{Overview}
We present our framework of a multi-view remote camera real-time (novel view synthesizing/3D reconstruction) simulation. 

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figs/poster.pdf}
    \caption{System model}
    \label{fig: poster}
\end{figure}

As shown in figure \ref{fig: poster}, the proposed framework considers a real-time multi-sensor streaming and edge reconstruction pipeline. The example in the figure illustrates a scenario where a wind turbine is being remotely inspected in a digital-twin way. To build the real-time digital twin, firstly, a team of autonomous robots, often consisting of \glspl{uav}, \glspl{ugv}, and quadruped robots, is sent to the scene of the incident. The robots will be distributed in a round formation at different height levels, trying to capture the information of the inspected object from all possible angles. The robot team will then start streaming real-time high-quality RGB images with camera poses through a wireless communication channel to a nearby \gls{bs}. The \gls{bs} is connected to edge servers with AI computing capability. 

In the considered system, the time is discretized into slots, and the duration of each slot is denoted by $T_s$. At the $t$-th timeslot, the image received by the server from the $i$-th robotic sensor is denoted by $x_i(t)$. Combining all the received data $x_i(t)$ at timeslot $t$ we have a set of images $X(t)$, which will then serve as the input of our reconstruction algorithm. 




% consists of two subsystems. Th



\subsection{Communication Model}
\cite{liu2007resource}
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figs/timeseries.pdf}
    \caption{Time Sequence Diagram}
    \label{fig: time}
\end{figure}

The proposed framework considers a time sequence of packets from each sensor to our edge server. 


To simulate the pattern of packet burstiness, we used the \gls{spp} \cite{hou2018burstiness} in our channel model, which will switch between a high-traffic state and a low-traffic state. In both states of the \gls{spp}, the packet arrival process is a Poisson process with either a high packet arrival rate $\lambda_H$, or a low packet arrival rate $\lambda_L$, so that the packet inter-arrival time $T_i$ in each state follows an exponential distribution:

\begin{equation}
        T_i^H \sim exp(\lambda_H), \; T_i^L \sim exp(\lambda_L)
\end{equation}

The communication delay $t_d$ as shown in Fig. 2, considered also in discrete time slots, follows an exponential distribution in both packet traffic states:

\begin{equation}
    T_d \sim exp(\lambda_d)
\end{equation}

Let $s_1$, and $s_2$ denote the low-traffic state and the high-traffic state, respectively. At any discrete time slot $t$, the switching of the two states is stochastic regarding the time from the last switching and the transition rate. The transition rate from state $s_1$ to state $s_2$ is denoted by $\lambda$, and the transition rate from the $s_2$ state to the $s_1$ state is represented as $\mu$. The generator matrix governing the transitions within this Markov chain is as follows:                                                                        
\begin{equation}
\begin{aligned}
     Q_s &= \begin{bmatrix}
        -\lambda & \lambda \\
        \mu & -\mu
        \end{bmatrix} \\
         &= \frac{1}{\lambda + \mu}
            \begin{bmatrix}
            1 & \lambda \\
            1 & -\mu
            \end{bmatrix}
            \begin{bmatrix}
            0 & 0 \\
            0 & -(\lambda+\mu)
            \end{bmatrix}
            \begin{bmatrix}
            \mu & \lambda \\
            1 & -1
            \end{bmatrix}.
\end{aligned}
\end{equation}


For consistency, the stationary distribution of the Markov chain should agree with the marginal distribution of the underlying channel
\begin{equation}
\label{eq2}
\begin{aligned}
   & P_r\{|h(t)| \leq \eta \} = \frac{\mu}{\lambda + \mu} = \int_0^{\eta} 2\xi e^{-\xi^2} d\xi = 1 - e^{-\eta^2} \\
   & P_r\{|h(t)| > \eta \} = \frac{\mu}{\lambda + \mu} = \int_{\eta}^{\infty} 2\xi e^{-\xi^2} d\xi = e^{-\eta^2}
\end{aligned}
\end{equation}

where $f(\xi)=2\xi e^{-\xi^2}$ with $\xi \geq 0$ is the marginal distribution of the normalized envelope process. To solve for $\lambda$ and $\mu$, two equations are needed. The first is given by condition (\ref{eq2}). The second condition can be derived from the Markov structure of the wireless link.

Let $P_t(t) = e^{Q_s t}$ be the probability transition matrix of the Gilbert-Elliot channel. More specifically, entry $p_{i,j}(t)$ of the matrix $P_t(t)$ represents the probability of being in state $j$ after $t$ seconds when starting in state $i$. For a time interval $t$, this probability transition matrix is given by
\begin{equation*}
    \begin{aligned}
        P_t(t) & = \frac{1}{\lambda + \mu}
            \begin{bmatrix}
            1 & \lambda \\
            1 & -\mu
            \end{bmatrix}
            \begin{bmatrix}
            0 & 0 \\
            0 & -(\lambda+\mu)
            \end{bmatrix}
            \begin{bmatrix}
            \mu & \lambda \\
            1 & -1
            \end{bmatrix} \\
            & = \frac{1}{\lambda + \mu}
            \begin{bmatrix}
                \mu+\lambda e^{-t(\lambda + \mu)} &
                \lambda-\lambda e^{-t(\lambda + \mu)} \\
                \mu-\mu e^{-t(\lambda + \mu)} &
                \lambda+\mu e^{-t(\lambda + \mu)} \\
            \end{bmatrix}.
    \end{aligned}
\end{equation*}




\subsection{The Instant Neural Graphics Primitives}

\gls{nerf} \cite{nerf} is a novel framework that has gained significant attention in recent years for its ability to revolutionize 3D scene representation and rendering. Traditional \gls{cv} techniques have been struggling to create 3D models of complex scenes and objects from 2D pictures, often requiring extensive manual modeling and texture mapping. \gls{nerf}, on the other hand, learn to infer scene geometry from synthesizing novel views directly from 2D images, enabling the generation of highly detailed and photorealistic 3D reconstructions.

\gls{nerf} models a 3D scene as a continuous function that maps 3D coordinates to 5D neural radiance values. This function is learned from a neural network that estimates the color and intensity of light at any point in the scene. This representation captures the geometry of the scene, including the position and orientation of objects, as well as their appearance. From this 3D reconstruction, \gls{nerf} also allows users to synthesize novel views of the scene from any desired perspective. By combining the learned 3D scene representation (kept as neural networks) with the camera parameters of the views, the algorithm can render images that are visually consistent with the real world. 

% Original Sentence from \cite{nerf} ===========================================
The neural radiance field interprets a scene as the volume density and directional emitted radiance at any perspective of view. With the classical volume rendering \cite{kajiya1984ray} method, the color of all rays passing through from a given input camera pose. The volume density, denoted as $\sigma(x)$, is viewed as the infinitesimal probability of a ray coming to an end at a minute particle situated at position $x$ \cite{nerf}. The expected color $C(\textbf{r})$ of camera ray $\textbf{r}(t) = \textbf{o} + t\textbf{d}$ with near and far bounds $t_n$ and $t_f$ is
\begin{equation}
\label{eq3}
    \begin{aligned}
        & C(\textbf{r}) = \int_{t_n}^{t_f} T(t)\sigma(\textbf{r}(t))\textbf{c}(\textbf{r}(t), \textbf{d})dt, \\
        & where \; T(t) = exp(-\int_{t_n}^{t}\sigma(\textbf{r}(s))ds
    \end{aligned}
\end{equation}

% Original Sentence from \cite{nerf} ===========================================
Instead of just using a single network to represent the scene, we simultaneously optimize two networks: one “coarse” and one “fine”. We first sample a set of $N_c$ locations using stratified sampling, and evaluate the “coarse” network at these locations as described in Eqns. 2 and (\ref{eq3}). Given the output of this “coarse” network, we then produce a more informed sampling of points along each ray where samples are biased towards the relevant parts of the volume. To do this, we first rewrite the alpha composited color from the coarse network $\hat{C}_c(\textbf{r})$ in Eqn. (\ref{eq3}) as a weighted sum of all sampled colors $c_i$ along the ray:
\begin{equation}
        \hat{C}_c(\textbf{r})=\sum_{i=1}^{N_c}w_i c_i, \; w_i = T_i(1-exp(-\sigma_i \delta_i))
\end{equation}
The loss is simply the total squared error between the rendered and true pixel colors for both the coarse and fine renderings:
\begin{equation}
    \mathcal{L} = \sum_{\textbf{r} \in \mathcal{R}} \lbrack {\lVert\hat{C}_c(\textbf{r}) - C(\textbf{r})\rVert}_2^2+{\lVert\hat{C}_f(\textbf{r}) - C(\textbf{r})\rVert}_2^2\rbrack 
\end{equation}

\gls{ngp} \cite{instantngp}


% Original Sentence from \cite{instantngp} ===========================================
Given a fully connected neural network $m(y; \phi)$, we are interested in an encoding of its inputs $y = enc(x; \theta)$ that improves the approximation quality and training speed across a wide range of applications without incurring a notable performance overhead. Our neural network not only has trainable weight parameters $\phi$ but also trainable encoding parameters $\theta$. These are arranged into $L$ levels, each containing up to $T$ feature vectors with dimensionality $F$. Typical values for these hyperparameters are shown in Table 1. Figure 3 illustrates the steps performed in our multiresolution hash encoding. Each level (two of which are shown as red and blue in the figure) is independent and conceptually stores feature vectors at the vertices of a grid, the resolution of which is chosen to be a geometric progression between the coarsest and finest resolutions $[N_{min}, N_{max}]$:

\begin{align}
     & N_l := [N_{min}\cdot b_l] \textcolor{red}{????} \\
     & b := -exp(\frac{\ln N_{max} - \ln N_{min}}{L-1}).
\end{align}

We use a spatial hash function \cite{teschner2003optimized} of the form
\begin{equation}
    h(x) = (\oplus_{i=1}^d x_i \pi_i) \mod T
\end{equation}
where $\oplus$ denotes the bit-wise XOR operation and $\pi_i$ are unique, large prime numbers. 

==> chapters/4_experimental_setup.tex <==
We are training our \gls{ngp} multi-view synthesis reconstruction model on the DyNeRF \cite{dyner} dataset. The dataset contains several 2704*2028 resolution 30 fps video from 19 synchronized cameras of around 40 seconds duration.

We choose \gls{psnr} as one of the KPIs to assess the fidelity and accuracy of the reconstruction or compression process. Let $I$, $K$ denote the image ground truth and the image to compare with, respectively. The \gls{psnr} \cite{jpeg} of $K$ compared to $I$ is defined as:
\begin{equation}
    \begin{aligned}
        & MSE = \frac{1}{mn}\sum_{i=0}^{m-1}\sum_{j=0}^{n-1}[I(i,j)-K(i,j)] \\
        & PSNR = 10 \cdot \log_{10}(\frac{{MAX}_I^2}{MSE})
    \end{aligned}
\end{equation}
where $I(i, j)$ denotes the $i$-th row by $j$-th column pixel value of the given image.

We choose \gls{ssim} as a metric to evaluate the degree of similarity between two images, considering their luminance, contrast, and structural information. Let $x$, $y$ denote the image ground truth and the image to compare with. Then the \gls{ssim} between $x$ and $y$ is defined as:
\begin{equation}
    \begin{aligned}
        & SSIM(x, y) = \frac{(2\mu_x\mu_y+c_1)(2\sigma_{xy}+c_2)}{(\mu_x^2+\mu_y^2+c_1)(\sigma_x^2+\sigma_y^2+c_2)} \\
        & c_1 = (k_1L)^2 \\
        & c_2 = (k_2L)^2 \\
    \end{aligned}
\end{equation}
where the pixel sample means of the images are denoted by $\mu_x$ and $\mu_y$, respectively; the variances of image $x$ and $y$ are denoted by $\sigma_x$ and $\sigma_y$, respectively; the covariance between $x$ and $y$ is $\sigma_{xy}$. $k_1$ and $k_2$ are small constants added to the denominator to avoid instability, often set to value 0.01 and 0.03, respectively. And image $x$, $y$ should have the same dynamic range $L$, often set to 255 for normal 8-bit images. 

\begin{figure}
            \centering
            \includegraphics[width=\linewidth]{figs/low_traffic.pdf}
           \caption{Novel view generation quality in low/high traffic state.}
           \label{fig: result}
\end{figure}

==> chapters/5_results.tex <==
\section{Results}






\subsection{Movements}



\subsection{Delay and burstiness}
\begin{table*}[t]\label{parameters}
\renewcommand{\arraystretch}{1.2}
\centering
\caption{Mean PSNR/SSIM with high/low communication delay}
\begin{threeparttable} 
\begin{tabular}{|l|l|l|l|l|l|l|l|l|}
% \hline 
% \multicolumn{2}{|c|}{\textbf{Prototype Setup}}  & \multicolumn{2}{c|}{\textbf{Learning Setup}} \\ 
\hline
\multirow{3}{*}{\textbf{Dataset}} & \multicolumn{4}{|c|}{\textbf{PSNR}} &\multicolumn{4}{|c|}{\textbf{SSIM}} \\
\cline{2-9}
 & \multicolumn{2}{|c|}{High Latency} & \multicolumn{2}{|c|}{Low Latency} & \multicolumn{2}{|c|}{High Latency} & \multicolumn{2}{|c|}{Low Latency}  \\
\cline{2-9}
& High Traffic  & Low Traffic & High Traffic  & Low Traffic & High Traffic  & Low Traffic & High Traffic  & Low Traffic\\
\hline
DyNeRF-Salmon & $30.59$ & $30.40$  & $30.40$  & $0.77$ & $0.77$ & $0.78$ & $30.59$ & $30.40$ \\
\hline
DyNeRF-Coffee & $30.59$ & $30.40$ & $30.40$  & $0.77$ & $0.77$ & $0.78$ & $30.59$ & $30.40$ \\
\hline
\end{tabular}
\end{threeparttable}
\label{tab:sys_param}
\end{table*}






\subsection{Methodology}
As shown in Table. \ref{t1}, we reconstructed the same datasets with 3 different state-of-the-art \gls{nerf} 3D reconstruction methods. Among which the k-planes and Nerfacto are both trained on the Nerfstudio \cite{nerfstudio}

\begin{table*}[t]\label{parameters}

\renewcommand{\arraystretch}{1.2}
\centering
\caption{Mean PSNR/SSIM with different reconstruction methods in high traffic state}
\begin{threeparttable} 
\label{t1}
\begin{tabular}{|l|l|l|l|l|l|l|}
% \hline 
% \multicolumn{2}{|c|}{\textbf{Prototype Setup}}  & \multicolumn{2}{c|}{\textbf{Learning Setup}} \\ 
\hline
\multirow{2}{*}{\textbf{Dataset}} & \multicolumn{3}{|c|}{\textbf{PSNR}} &\multicolumn{3}{|c|}{\textbf{SSIM}} \\
\cline{2-7}
 & Instant-NGP & K-Planes & Nerfacto  & Instant-NGP & K-Planes & Nerfacto\\
\hline
DyNeRF-Salmon & $30.59$ & $30.40$  & $30.40$  & $0.77$ & $0.77$ & $0.78$ \\
\hline
DyNeRF-Coffee & $30.59$ & $30.40$ & $30.40$  & $0.77$ & $0.77$ & $0.78$ \\
\hline
\end{tabular}
\end{threeparttable}
\label{tab:sys_param}
\end{table*}


% \subsection{Burstiness}
% \begin{table*}[t]\label{parameters}
% \renewcommand{\arraystretch}{1.2}
% \centering
% \caption{Mean PSNR/SSIM under high/low traffic states with Instant-NGP}
% \begin{threeparttable} 
% \begin{tabular}{|l|l|l|l|l|}
% % \hline 
% % \multicolumn{2}{|c|}{\textbf{Prototype Setup}}  & \multicolumn{2}{c|}{\textbf{Learning Setup}} \\ 
% \hline
% \multirow{2}{*}{\textbf{Dataset}} & \multicolumn{2}{|c|}{\textbf{PSNR}} &\multicolumn{2}{|c|}{\textbf{SSIM}} \\
% \cline{2-5}
%  & High Traffic & Low Traffic &High Traffic &Low Traffic\\
% \hline
% DyNeRF\cite{dynerf}-Salmon & $30.59$ & $30.40$  & $0.77$ & $0.78$\\
% \hline
% DyNeRF-Coffee & $30.59$ & $30.40$  & $0.77$ & $0.78$\\
% \hline
% \end{tabular}
% \end{threeparttable}
% \label{tab:sys_param}
% \end{table*}

==> chapters/6_conclusion.tex <==
\section{Conclusion}
In this paper, we established a framework for evaluating the effects of packet burstiness and communication latency on the real-time 3D reconstruction. 






1. Once high traffic states occur and the reconstruction is in low-quality, the low-quality mode will last longer than the high traffic state and need the channel to be in low traffic state for some time to recover
